Safely: Safe Stochastic Motion Planning Under Constrained Sensing via Duality

Consider a robot operating in an uncertain environment with stochastic, dynamic obstacles. Despite the clear benefits for trajectory optimization, it is often hard to keep track of each obstacle at every time step due to sensing and hardware limitations. We introduce the Safely motion planner, a receding-horizon control framework, that simultaneously synthesizes both a trajectory for the robot to follow as well as a sensor selection strategy that prescribes trajectory-relevant obstacles to measure at each time step while respecting the sensing constraints of the robot. We perform the motion planning using sequential quadratic programming, and prescribe obstacles to sense based on the duality information associated with the convex subproblems. We guarantee safety by ensuring that the probability of the robot colliding with any of the obstacles is below a prescribed threshold at every time step of the planned robot trajectory. We demonstrate the efficacy of the Safely motion planner through software and hardware experiments.

==> figure_motionplans.tex <==
%
% \begin{figure}[t]
%     \centering
%     \includegraphics{updated_experimental_results/experiment_1/ICRA_2021_Safety_and_Attention.pdf}
%     \caption{Initial configuration of the simulation. The blue dot is the initial position of the robot, the yellow dot is the target state, and the red-shaded regions are the combined hard-body shapes of the robot and the obstacles.}
%     \label{fig:example_env}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \scalebox{0.75}{
        \includegraphics{updated_experimental_results/experiment_1/3d_init_config_new.pdf}}
        \caption{Initial configuration of Example 1.}
        \label{fig:example_env}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
        \scalebox{1}{
        \includegraphics{updated_experimental_results/experiment_2/updated_obstacle_init_pos.pdf}}
        \caption{Initial configuration of Example 2.}
        \label{fig:nonlin_example_env}
    \end{subfigure}
    \caption{Initial configurations of the sample environments.}
    %
    \label{fig:simulation_init_configs}
\end{figure}

% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering        
%         \scalebox{0.4}{\includestandalone{sum_plot_six_files/sum_fig_12_clipped}}
%         \caption{$t=12$, $\algName$}
%         \label{fig:sum_10}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%     \centering
%         \scalebox{0.2}{\includestandalone{sum_plot_six_files/sum_fig_20_clipped}}
%         \caption{$t=20$, $\algName$}
%         \label{fig:sum_20}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{sum_plot_six_files/sum_fig_28_clipped}}
%         \caption{$t=28$, $\algName$}
%         \label{fig:sum_30}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{sum_plot_six_files/sum_fig_36_clipped}}
%         \caption{$t=36$, $\algName$}
%         \label{fig:sum_40}
%     \end{subfigure}
%     %
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{bin_plot_six_files/bin_fig_12_clipped}}
%         \caption{$t=12$, \texttt{binning}}
%         \label{fig:bin_10}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{bin_plot_six_files/bin_fig_20_clipped}}
%         \caption{$t=20$, \texttt{binning}}
%         \label{fig:bin_20}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{bin_plot_six_files/bin_fig_28_clipped}}
%         \caption{$t=28$, \texttt{binning}}
%         \label{fig:bin_30}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \scalebox{0.2}{
%         \includestandalone{bin_plot_six_files/bin_fig_36_clipped}}
%         \caption{$t=36$, \texttt{binning}}
%         \label{fig:bin_40}
%     \end{subfigure}
%     %
%     \caption{Comparison of trajectories based on sensor selection strategy considered --- \algName{} (a) -- (d) vs the alternative \texttt{binning} strategy (e) -- (h). The black marks indicate the trajectory of the robot up to the current time step, while the light blue marks indicate the future motion plan. The red marks indicate the realization of the random obstacle trajectories up to the current time step. The ellipsoids indicate the keep-out regions for guaranteeing probabilistic safety (Proposition~\ref{prop:1}). The obstacle ellipsoid selected for observation at a particular time step is colored blue, and otherwise is colored red. }
%     % We plot the keep-out ellipsoids for previous $14$ time steps for each obstacle with decreasing opacity.
%     % planned trajectory of the robot for the following $T$ time steps
%     % The ellipsoids $\mathcal{E}(\mu_{o}[t],Q_{o}^{+}[t])$ for each obstacle are plotted for the current time step, while the ellipsoids corresponding to the previous $14$ time steps are plotted with a decreasing opacity. 
%     %
%     \label{fig:plot_traj}
% \end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering        
        \scalebox{2.25}{\includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_10_new.pdf}}
        \caption{$t=10$}
        \label{fig:sum_10}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
        \scalebox{2.25}{\includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_20_new.pdf}}
        \caption{$t=20$}
        \label{fig:sum_20}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \scalebox{2.25}{
        \includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_30_new.pdf}}
        \caption{$t=30$}
        \label{fig:sum_30}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \scalebox{2.25}{
        \includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_40_new.pdf}}
        \caption{$t=40$}
        \label{fig:sum_40}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \scalebox{2.25}{
        \includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_50_new.pdf}}
        \caption{$t=50$}
        \label{fig:sum_50}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \scalebox{2.25}{
        \includegraphics{updated_experimental_results/experiment_1/env_time_steps/3d_time_60_new.pdf}}
        \caption{$t=60$}
        \label{fig:sum_60}
    \end{subfigure}
    %
    \caption{Trajectory obtained using the \algName{} motion planner at various time steps over the simulation. The black marks indicate the trajectory of the robot up to the current time step, while the light blue marks indicate the future motion plan. The red marks indicate the realization of the random obstacle trajectories up to the current time step. The ellipsoids indicate the keep-out regions for guaranteeing probabilistic safety (Proposition~\ref{prop:1}). The obstacle ellipsoid selected for observation at a particular time step is colored blue, and otherwise is colored red. }
    %
    \label{fig:plot_traj}
\end{figure*}
